Essential Incompleteness of Arithmetic Verified by Coq

A constructive proof of the Goedel-Rosser incompleteness theorem has been completed using the Coq proof assistant. Some theory of classical first-order logic over an arbitrary language is formalized. A development of primitive recursive functions is given, and all primitive recursive functions are proved to be representable in a weak axiom system. Formulas and proofs are encoded as natural numbers, and functions operating on these codes are proved to be primitive recursive. The weak axiom system is proved to be essentially incomplete. In particular, Peano arithmetic is proved to be consistent in Coq's type theory and therefore is incomplete.

==> Goedel/Makefile <==
##############################################################################
##                 The Calculus of Inductive Constructions                  ##
##                                                                          ##
##                                Projet Coq                                ##
##                                                                          ##
##                     INRIA                        ENS-CNRS                ##
##              Rocquencourt                        Lyon                    ##
##                                                                          ##
##                                  Coq V7                                  ##
##                                                                          ##
##                                                                          ##
##############################################################################

# WARNING
#
# This Makefile has been automagically generated by coq_makefile
# Edit at your own risks !
#
# END OF WARNING

#
# This Makefile was generated by the command line :
# coq_makefile -f Make -o Makefile 
#

##########################
#                        #
# Variables definitions. #
#                        #
##########################

CAMLP4LIB=`camlp4 -where`
COQSRC=-I $(COQTOP)/kernel -I $(COQTOP)/lib \
  -I $(COQTOP)/library -I $(COQTOP)/parsing \
  -I $(COQTOP)/pretyping -I $(COQTOP)/interp \
  -I $(COQTOP)/proofs -I $(COQTOP)/syntax -I $(COQTOP)/tactics \
  -I $(COQTOP)/toplevel -I $(COQTOP)/contrib/correctness \
  -I $(COQTOP)/contrib/extraction -I $(COQTOP)/contrib/field \
  -I $(COQTOP)/contrib/fourier -I $(COQTOP)/contrib/graphs \
  -I $(COQTOP)/contrib/interface -I $(COQTOP)/contrib/jprover \
  -I $(COQTOP)/contrib/omega -I $(COQTOP)/contrib/romega \
  -I $(COQTOP)/contrib/ring -I $(COQTOP)/contrib/xml \
  -I $(CAMLP4LIB)
ZFLAGS=$(OCAMLLIBS) $(COQSRC)
OPT=
COQFLAGS=-q $(OPT) $(COQLIBS) $(OTHERFLAGS) $(COQ_XML)
COQC=$(COQBIN)coqc
GALLINA=gallina
COQDOC=coqdoc
CAMLC=ocamlc -c
CAMLOPTC=ocamlopt -c
CAMLLINK=ocamlc
CAMLOPTLINK=ocamlopt
COQDEP=$(COQBIN)coqdep -c
GRAMMARS=grammar.cma
CAMLP4EXTEND=pa_extend.cmo pa_ifdef.cmo q_MLast.cmo
PP=-pp "camlp4o -I . -I $(COQTOP)/parsing $(CAMLP4EXTEND) $(GRAMMARS) -impl"

#########################
#                       #
# Libraries definition. #
#                       #
#########################

OCAMLLIBS=-I .\
  -I POCKLINGTON
COQLIBS=-I .\
  -I POCKLINGTON

###################################
#                                 #
# Definition of the "all" target. #
#                                 #
###################################

VFILES=Deduction.v\
  LNN.v\
  LNN2LNT.v\
  LNT.v\
  Languages.v\
  ListExt.v\
  NN.v\
  NN2PA.v\
  NNtheory.v\
  PA.v\
  PAconsistent.v\
  PAtheory.v\
  PRrepresentable.v\
  cPair.v\
  chRem.v\
  checkPrf.v\
  code.v\
  codeFreeVar.v\
  codeList.v\
  codeNatToTerm.v\
  codePA.v\
  codeSubFormula.v\
  codeSubTerm.v\
  codeSysPrf.v\
  expressible.v\
  extEqualNat.v\
  fixPoint.v\
  fol.v\
  folLogic.v\
  folLogic2.v\
  folLogic3.v\
  folProof.v\
  folProp.v\
  folReplace.v\
  godel1.v\
  misc.v\
  model.v\
  prLogic.v\
  primRec.v\
  rosser.v\
  rosserPA.v\
  subAll.v\
  subProp.v\
  vector.v\
  wConsistent.v\
  wellFormed.v
VOFILES=$(VFILES:.v=.vo)
VIFILES=$(VFILES:.v=.vi)
GFILES=$(VFILES:.v=.g)
HTMLFILES=$(VFILES:.v=.html)
GHTMLFILES=$(VFILES:.v=.g.html)

all: Deduction.vo\
  LNN.vo\
  LNN2LNT.vo\
  LNT.vo\
  Languages.vo\
  ListExt.vo\
  NN.vo\
  NN2PA.vo\
  NNtheory.vo\
  PA.vo\
  PAconsistent.vo\
  PAtheory.vo\
  PRrepresentable.vo\
  cPair.vo\
  chRem.vo\
  checkPrf.vo\
  code.vo\
  codeFreeVar.vo\
  codeList.vo\
  codeNatToTerm.vo\
  codePA.vo\
  codeSubFormula.vo\
  codeSubTerm.vo\
  codeSysPrf.vo\
  expressible.vo\
  extEqualNat.vo\
  fixPoint.vo\
  fol.vo\
  folLogic.vo\
  folLogic2.vo\
  folLogic3.vo\
  folProof.vo\
  folProp.vo\
  folReplace.vo\
  godel1.vo\
  misc.vo\
  model.vo\
  prLogic.vo\
  primRec.vo\
  rosser.vo\
  rosserPA.vo\
  subAll.vo\
  subProp.vo\
  vector.vo\
  wConsistent.vo\
  wellFormed.vo

spec: $(VIFILES)

gallina: $(GFILES)

html: $(HTMLFILES)

gallinahtml: $(GHTMLFILES)

all.ps: $(VFILES)
	$(COQDOC) -ps -o $@ `$(COQDEP) -sort -suffix .v $(VFILES)`

all-gal.ps: $(VFILES)
	$(COQDOC) -ps -g -o $@ `$(COQDEP) -sort -suffix .v $(VFILES)`



####################
#                  #
# Special targets. #
#                  #
####################

.PHONY: all opt byte archclean clean install depend html

.SUFFIXES: .v .vo .vi .g .html .tex .g.tex .g.html

.v.vo:
	$(COQC) $(COQDEBUG) $(COQFLAGS) $*

.v.vi:
	$(COQC) -i $(COQDEBUG) $(COQFLAGS) $*

.v.g:
	$(GALLINA) $<

.v.tex:
	$(COQDOC) -latex $< -o $@

.v.html:
	$(COQDOC) -html $< -o $@

.v.g.tex:
	$(COQDOC) -latex -g $< -o $@

.v.g.html:
	$(COQDOC) -html -g $< -o $@

byte:
	$(MAKE) all "OPT="

opt:
	$(MAKE) all "OPT=-opt"

include .depend

.depend depend:
	rm -f .depend
	$(COQDEP) -i $(COQLIBS) *.v *.ml *.mli >.depend
	$(COQDEP) $(COQLIBS) -suffix .html *.v >>.depend

install:
	mkdir -p `$(COQC) -where`/user-contrib
	cp -f *.vo `$(COQC) -where`/user-contrib

Makefile: Make
	mv -f Makefile Makefile.bak
	$(COQBIN)coq_makefile -f Make -o Makefile


clean:
	rm -f *.cmo *.cmi *.cmx *.o *.vo *.vi *.g *~
	rm -f all.ps all-gal.ps $(HTMLFILES) $(GHTMLFILES)

archclean:
	rm -f *.cmx *.o

html:

# WARNING
#
# This Makefile has been automagically generated by coq_makefile
# Edit at your own risks !
#
# END OF WARNING



==> Goedel/POCKLINGTON/Makefile <==
##############################################################################
##                 The Calculus of Inductive Constructions                  ##
##                                                                          ##
##                                Projet Coq                                ##
##                                                                          ##
##                     INRIA                        ENS-CNRS                ##
##              Rocquencourt                        Lyon                    ##
##                                                                          ##
##                                  Coq V7                                  ##
##                                                                          ##
##                                                                          ##
##############################################################################

# WARNING
#
# This Makefile has been automagically generated by coq_makefile
# Edit at your own risks !
#
# END OF WARNING

#
# This Makefile was generated by the command line :
# coq_makefile -f Make -o Makefile 
#

##########################
#                        #
# Variables definitions. #
#                        #
##########################

CAMLP4LIB=`camlp4 -where`
COQSRC=-I $(COQTOP)/kernel -I $(COQTOP)/lib \
  -I $(COQTOP)/library -I $(COQTOP)/parsing \
  -I $(COQTOP)/pretyping -I $(COQTOP)/interp \
  -I $(COQTOP)/proofs -I $(COQTOP)/syntax -I $(COQTOP)/tactics \
  -I $(COQTOP)/toplevel -I $(COQTOP)/contrib/correctness \
  -I $(COQTOP)/contrib/extraction -I $(COQTOP)/contrib/field \
  -I $(COQTOP)/contrib/fourier -I $(COQTOP)/contrib/graphs \
  -I $(COQTOP)/contrib/interface -I $(COQTOP)/contrib/jprover \
  -I $(COQTOP)/contrib/omega -I $(COQTOP)/contrib/romega \
  -I $(COQTOP)/contrib/ring -I $(COQTOP)/contrib/xml \
  -I $(CAMLP4LIB)
ZFLAGS=$(OCAMLLIBS) $(COQSRC)
OPT=
COQFLAGS=-q $(OPT) $(COQLIBS) $(COQ_XML)
COQC=$(COQBIN)coqc
GALLINA=gallina
COQDOC=coqdoc
CAMLC=ocamlc -c
CAMLOPTC=ocamlopt -c
CAMLLINK=ocamlc
CAMLOPTLINK=ocamlopt
COQDEP=$(COQBIN)coqdep -c
COQVO2XML=coq_vo2xml
GRAMMARS=grammar.cma
CAMLP4EXTEND=pa_extend.cmo pa_ifdef.cmo q_MLast.cmo
PP=-pp "camlp4o -I . -I $(COQTOP)/parsing $(CAMLP4EXTEND) $(GRAMMARS) -impl"

#########################
#                       #
# Libraries definition. #
#                       #
#########################

OCAMLLIBS=-I .
COQLIBS=-I .

###################################
#                                 #
# Definition of the "all" target. #
#                                 #
###################################

VFILES=Pocklington.v\
  dec.v\
  divides.v\
  exp.v\
  fermat.v\
  gcd.v\
  lemmas.v\
  list.v\
  modulo.v\
  modprime.v\
  natZ.v\
  order.v\
  pock.v\
  prime.v
VOFILES=$(VFILES:.v=.vo)
VIFILES=$(VFILES:.v=.vi)
GFILES=$(VFILES:.v=.g)
HTMLFILES=$(VFILES:.v=.html)
GHTMLFILES=$(VFILES:.v=.g.html)

all: Pocklington.vo\
  dec.vo\
  divides.vo\
  exp.vo\
  fermat.vo\
  gcd.vo\
  lemmas.vo\
  list.vo\
  modulo.vo\
  modprime.vo\
  natZ.vo\
  order.vo\
  pock.vo\
  prime.vo

spec: $(VIFILES)

gallina: $(GFILES)

html: $(HTMLFILES)

gallinahtml: $(GHTMLFILES)

all.ps: $(VFILES)
	$(COQDOC) -ps -o $@ `$(COQDEP) -sort -suffix .v $(VFILES)`

all-gal.ps: $(VFILES)
	$(COQDOC) -ps -g -o $@ `$(COQDEP) -sort -suffix .v $(VFILES)`

xml:: .xml_time_stamp
.xml_time_stamp: Pocklington.vo\
  dec.vo\
  divides.vo\
  exp.vo\
  fermat.vo\
  gcd.vo\
  lemmas.vo\
  list.vo\
  modulo.vo\
  modprime.vo\
  natZ.vo\
  order.vo\
  pock.vo\
  prime.vo
	$(COQVO2XML) $(COQFLAGS) $(?:%.o=%)
	touch .xml_time_stamp

####################
#                  #
# Special targets. #
#                  #
####################

.PHONY: all opt byte archclean clean install depend xml

.SUFFIXES: .v .vo .vi .g .html .tex .g.tex .g.html

.v.vo:
	$(COQC) $(COQDEBUG) $(COQFLAGS) $*

.v.vi:
	$(COQC) -i $(COQDEBUG) $(COQFLAGS) $*

.v.g:
	$(GALLINA) $<

.v.tex:
	$(COQDOC) -latex $< -o $@

.v.html:
	$(COQDOC) -html $< -o $@

.v.g.tex:
	$(COQDOC) -latex -g $< -o $@

.v.g.html:
	$(COQDOC) -html -g $< -o $@

byte:
	$(MAKE) all "OPT="

opt:
	$(MAKE) all "OPT=-opt"

include .depend

depend:
	rm .depend
	$(COQDEP) -i $(COQLIBS) *.v *.ml *.mli >.depend
	$(COQDEP) $(COQLIBS) -suffix .html *.v >>.depend

xml::

install:
	mkdir -p `$(COQC) -where`/user-contrib
	cp -f *.vo `$(COQC) -where`/user-contrib

Makefile: Make
	mv -f Makefile Makefile.bak
	$(COQBIN)coq_makefile -f Make -o Makefile

clean:
	rm -f *.cmo *.cmi *.cmx *.o *.vo *.vi *.g *~
	rm -f all.ps all-gal.ps $(HTMLFILES) $(GHTMLFILES)

archclean:
	rm -f *.cmx *.o

# WARNING
#
# This Makefile has been automagically generated by coq_makefile
# Edit at your own risks !
#
# END OF WARNING


